Spinning switches on a wreath product

We classify an algebraic phenomenon on certain families of wreath products that can be seen as coming from a family of puzzles about switches on the corners of a spinning table. Such puzzles have been written about and generalized since they were first popularized by Martin Gardner in 1979. In this paper, we provide perhaps the fullest generalization yet, modeling both the switches and the spinning table as arbitrary finite groups combined via a wreath product. We classify large families of wreath products depending on whether or not they correspond to a solvable puzzle, completely classifying the puzzle in the case when the switches behave like abelian groups, constructing winning strategies for all wreath product that are $p$-groups, and providing novel examples for other puzzles where the switches behave like nonabelian groups, including the puzzle consisting of two interchangeable copies of the monster group $M$. Lastly, we provide a number of open questions and conjectures, and provide other suggestions of how to generalize some of these ideas further.

==> assets/fig_derangementPrefix.tex <==
\begin{figure}
  \center
  \begin{tikzpicture}[scale = 0.5]
    \path (0,-0.5) -- (0,6.5);
    \foreach \i in {0,...,11} { \fill[gray] (\i, 12-\i) rectangle (\i + 1, 11 - \i); }
    \draw (0,0) grid (12,12);
    \node (R1) at (5.5, 11.5) {\Large\rook};
    \node (R2) at (0.5, 10.5) {\Large\rook};
    \draw[line width = 3]
      (0.5,11.5) -- (R1) -- (11.5,11.5)
      (R1) -- (5.5,0.5)
    ;
    \draw[line width = 3]
      (R2) -- (11.5,10.5)
      (R2) -- (0.5,0.5)
    ;
  \end{tikzpicture}
  ~~
  \begin{tikzpicture}[scale = 0.5]
    \path (0,-0.5) -- (0,6.5);
    \foreach \i in {1,...,3} { \fill[gray] (\i, 11-\i) rectangle (\i + 1, 10 - \i); }
    \foreach \i in {4,...,9} { \fill[gray] (\i, 10-\i) rectangle (\i + 1, 9 - \i); }
    \draw (0,0) grid (10,10);
  \end{tikzpicture}
  \caption[The derived board for a prefix of a derangement.]{An example of a prefix $\alpha = (6, 1)$, and the board that results
  from deleting the first $\ell = 2$ rows and columns $6$ and $1$.
  The derived complementary board of $B$ from $\alpha$ is
  $B^c_\alpha = \{(1,2), (2,3), (3,4), (5,5), \dots, (10,10)\}$.}
\label{fig:derangementPrefix}
\end{figure}

